WordNet2Vec: Corpora Agnostic Word Vectorization Method

A complex nature of big data resources demands new methods for structuring especially for textual content. WordNet is a good knowledge source for comprehensive abstraction of natural language as its good implementations exist for many languages. Since WordNet embeds natural language in the form of a complex network, a transformation mechanism WordNet2Vec is proposed in the paper. It creates vectors for each word from WordNet. These vectors encapsulate general position - role of a given word towards all other words in the natural language. Any list or set of such vectors contains knowledge about the context of its component within the whole language. Such word representation can be easily applied to many analytic tasks like classification or clustering. The usefulness of the WordNet2Vec method was demonstrated in sentiment analysis, i.e. classification with transfer learning for the real Amazon opinion textual dataset.

==> transfer-wordnet-12-3-45.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% wordnet2vec results
AUTOMOTIVE
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.7285448578417829
Recall = 0.7285448578417829
F1 Score = 0.7285448578417829
Precision(0.0) = 0.5200206805534769                                             
Precision(1.0) = 0.1570632862767694
Precision(2.0) = 0.7830838536252176
Recall(0.0) = 0.32831397746014296
Recall(1.0) = 0.06883996969441872
Recall(2.0) = 0.9099554967972591
FPR(0.0) = 0.07393513123810641
FPR(1.0) = 0.03214918834974215
FPR(2.0) = 0.6605970768367372
F1-Score(0.0) = 0.40250638443514203
F1-Score(1.0) = 0.09572444470457404
F1-Score(2.0) = 0.8417659718087873
Weighted precision: 0.6813749298453917
Weighted recall: 0.7285448578417828
Weighted F1 score: 0.695891637574275
Weighted false positive rate: 0.4952262542663686
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7260616907758357
Recall = 0.7260616907758357
F1 Score = 0.7260616907758357
Precision(0.0) = 0.22826835652293703                                            
Precision(1.0) = 0.14982529699510833
Precision(2.0) = 0.8274219988348935
Recall(0.0) = 0.24707987474526566
Recall(1.0) = 0.0717104823065088
Recall(2.0) = 0.8633048271962683
FPR(0.0) = 0.10742845454138673
FPR(1.0) = 0.03764023043271105
FPR(2.0) = 0.7265027945705487
F1-Score(0.0) = 0.23730189039526448
F1-Score(1.0) = 0.09699601882012306
F1-Score(2.0) = 0.8449826367271268
Weighted precision: 0.7017762324268169
Weighted recall: 0.7260616907758358
Weighted F1 score: 0.7124053483202433
Weighted false positive rate: 0.5976331703204822
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7764012582006714
Recall = 0.7764012582006714
F1 Score = 0.7764012582006714
Precision(0.0) = 0.19623258108274758                                            
Precision(1.0) = 0.13307500398110303
Precision(2.0) = 0.8560215707610574
Recall(0.0) = 0.19989322278751334
Recall(1.0) = 0.049770701395644316
Recall(2.0) = 0.8997083636070073
FPR(0.0) = 0.08084695331554376
FPR(1.0) = 0.0248108650077477
FPR(2.0) = 0.788873788961466
F1-Score(0.0) = 0.19804598774075113
F1-Score(1.0) = 0.07244617829793382
F1-Score(2.0) = 0.877321450828867
Weighted precision: 0.7453383752277736
Weighted recall: 0.7764012582006714
Weighted F1 score: 0.7590633574855625
Weighted false positive rate: 0.6709328654854289
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.7410977675427745
Recall = 0.7410977675427745
F1 Score = 0.7410977675427745
Precision(0.0) = 0.43340336134453783                                            
Precision(1.0) = 0.18128528006947459
Precision(2.0) = 0.8115432377511854
Recall(0.0) = 0.2984750716166556
Recall(1.0) = 0.10433587404723228
Recall(2.0) = 0.9007938248322442
FPR(0.0) = 0.07678816488528753
FPR(1.0) = 0.03884305182163716
FPR(2.0) = 0.6602788490062296
F1-Score(0.0) = 0.35350160215219595
F1-Score(1.0) = 0.13244507891188834
F1-Score(2.0) = 0.8538425677100191
Weighted precision: 0.7013665973833401
Weighted recall: 0.7410977675427746
Weighted F1 score: 0.7166312758423313
Weighted false positive rate: 0.5170078332559287
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6699954882088189
Recall = 0.6699954882088189
F1 Score = 0.6699954882088189
Precision(0.0) = 0.34352110800372887                                            
Precision(1.0) = 0.15213808656431607
Precision(2.0) = 0.7825382897824955
Recall(0.0) = 0.33404558404558404
Recall(1.0) = 0.101270207852194
Recall(2.0) = 0.821466548847519
FPR(0.0) = 0.13070569674793514
FPR(1.0) = 0.05944923552236264
FPR(2.0) = 0.6323431795552605
F1-Score(0.0) = 0.3387170901450988
F1-Score(1.0) = 0.1215986689313321
F1-Score(2.0) = 0.8015300362780808
Weighted precision: 0.6478509006211306
Weighted recall: 0.6699954882088188
Weighted F1 score: 0.6580783093481829
Weighted false positive rate: 0.49249360003437725
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7161789355598731
Recall = 0.7161789355598731
F1 Score = 0.7161789355598731
Precision(0.0) = 0.28245977736716393                                            
Precision(1.0) = 0.15957806477787545
Precision(2.0) = 0.8011879350348028
Recall(0.0) = 0.24136868657693566
Recall(1.0) = 0.06799389207410182
Recall(2.0) = 0.875611529033894
FPR(0.0) = 0.09635262221469118
FPR(1.0) = 0.03574551060084899
FPR(2.0) = 0.7417418803813393
F1-Score(0.0) = 0.26030256149349507
F1-Score(1.0) = 0.09535738817730009
F1-Score(2.0) = 0.8367481119502443
Weighted precision: 0.6725096953150695
Weighted recall: 0.7161789355598731
Weighted F1 score: 0.691175406230296
Weighted false positive rate: 0.5900189487567525
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7526477517156611
Recall = 0.7526477517156611
F1 Score = 0.7526477517156611
Precision(0.0) = 0.4058518168947617                                             
Precision(1.0) = 0.19807008633824277
Precision(2.0) = 0.8158275006987268
Recall(0.0) = 0.30218911416423627
Recall(1.0) = 0.07120686507211978
Recall(2.0) = 0.9123628383321141
FPR(0.0) = 0.07547916379398205
FPR(1.0) = 0.026488992277538877
FPR(2.0) = 0.6899309423034083
F1-Score(0.0) = 0.3464319523051824
F1-Score(1.0) = 0.10475423045930701
F1-Score(2.0) = 0.8613989759302804
Weighted precision: 0.7040899709397687
Weighted recall: 0.7526477517156611
Weighted F1 score: 0.7226717592029412
Weighted false positive rate: 0.5445468500905905
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.7534480911519441
Recall = 0.7534480911519441
F1 Score = 0.7534480911519441
Precision(0.0) = 0.3683840278708294                                             
Precision(1.0) = 0.24572587655751957
Precision(2.0) = 0.8287553875143973
Recall(0.0) = 0.28141153590255386
Recall(1.0) = 0.13341724354940215
Recall(2.0) = 0.9055861176460124
FPR(0.0) = 0.07533411910422119
FPR(1.0) = 0.039448508935776824
FPR(2.0) = 0.6523208582679607
F1-Score(0.0) = 0.31907732482228346
F1-Score(1.0) = 0.17293769756296523
F1-Score(2.0) = 0.8654689651655021
Weighted precision: 0.7153568732651014
Weighted recall: 0.7534480911519441
Weighted F1 score: 0.730832513826322
Weighted false positive rate: 0.5205515774599029
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.7598964274577756
Recall = 0.7598964274577756
F1 Score = 0.7598964274577756
Precision(0.0) = 0.3948309848872016                                             
Precision(1.0) = 0.21316418841634605
Precision(2.0) = 0.8304273867743993
Recall(0.0) = 0.3181176470588235
Recall(1.0) = 0.09577201588413922
Recall(2.0) = 0.9075950773956271
FPR(0.0) = 0.07557818818412666
FPR(1.0) = 0.03262425413030732
FPR(2.0) = 0.6621243570074903
F1-Score(0.0) = 0.3523471348991758
F1-Score(1.0) = 0.1321642705176971
F1-Score(2.0) = 0.8672981206038399
Weighted precision: 0.7198179254186455
Weighted recall: 0.7598964274577756
Weighted F1 score: 0.7360804186391491
Weighted false positive rate: 0.5302232267797
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.7810200375903922
Recall = 0.7810200375903922
F1 Score = 0.7810200375903922
Precision(0.0) = 0.49470134874759153                                            
Precision(1.0) = 0.26682224815246985
Precision(2.0) = 0.8338873704168821
Recall(0.0) = 0.3591411386207861
Recall(1.0) = 0.09929078014184398
Recall(2.0) = 0.9282405503933339
FPR(0.0) = 0.06566510172143974
FPR(1.0) = 0.021601118445177852
FPR(2.0) = 0.6362050266421465
F1-Score(0.0) = 0.4161601426371667
F1-Score(1.0) = 0.14472573839662448
F1-Score(2.0) = 0.8785378888110618
Weighted precision: 0.7407870691887982
Weighted recall: 0.7810200375903921
Weighted F1 score: 0.754500371029875
Weighted false positive rate: 0.5044912843991562
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!




MOVIES
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6420941970874244
Recall = 0.6420941970874244
F1 Score = 0.6420941970874244
Precision(0.0) = 0.3420868401810856                                             
Precision(1.0) = 0.12622935791830908
Precision(2.0) = 0.7716438077911526
Recall(0.0) = 0.1888829714128642
Recall(1.0) = 0.20285798467884503
Recall(2.0) = 0.8134775808133472
FPR(0.0) = 0.08863078122511255
FPR(1.0) = 0.12219072315986873
FPR(2.0) = 0.6309201376180368
F1-Score(0.0) = 0.243382495365118
F1-Score(1.0) = 0.1556221090275031
F1-Score(2.0) = 0.792008665739058
Weighted precision: 0.635727854429002
Weighted recall: 0.6420941970874244
Weighted F1 score: 0.6334623120535939
Weighted false positive rate: 0.4838358390904425
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7120946091369408
Recall = 0.7120946091369408
F1 Score = 0.7120946091369408
Precision(0.0) = 0.2819664998912334                                             
Precision(1.0) = 0.1584804079543516
Precision(2.0) = 0.853021126252794
Recall(0.0) = 0.16106665341219742
Recall(1.0) = 0.27961736571008095
Recall(2.0) = 0.8361403632765566
FPR(0.0) = 0.052748994815870726
FPR(1.0) = 0.13734074216163702
FPR(2.0) = 0.5812849321318581
F1-Score(0.0) = 0.2050203248817677
F1-Score(1.0) = 0.20230129826132198
F1-Score(2.0) = 0.8444963951745306
Weighted precision: 0.7291426431163083
Weighted recall: 0.7120946091369408
Weighted F1 score: 0.717253259423244
Weighted false positive rate: 0.4834692782463067
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7752511532800569
Recall = 0.7752511532800569
F1 Score = 0.7752511532800569
Precision(0.0) = 0.24504214874488328                                            
Precision(1.0) = 0.15637934137124349
Precision(2.0) = 0.8732790518197308
Recall(0.0) = 0.20586018466176748
Recall(1.0) = 0.1552679120922753
Recall(2.0) = 0.8887610667097225
FPR(0.0) = 0.06262685150872863
FPR(1.0) = 0.0640962537599125
FPR(2.0) = 0.6723159879005742
F1-Score(0.0) = 0.2237487733071639
F1-Score(1.0) = 0.1558216448836468
F1-Score(2.0) = 0.8809520435644786
Weighted precision: 0.7658612359883328
Weighted recall: 0.7752511532800569
Weighted F1 score: 0.7703459927777941
Weighted false positive rate: 0.5742902464492723
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.6637040138553185
Recall = 0.6637040138553185
F1 Score = 0.6637040138553185
Precision(0.0) = 0.3004484304932735                                             
Precision(1.0) = 0.13901451231859602
Precision(2.0) = 0.8145897234403914
Recall(0.0) = 0.1977487774530513
Recall(1.0) = 0.2573409971260777
Recall(2.0) = 0.8053468832820616
FPR(0.0) = 0.09060832626286208
FPR(1.0) = 0.13138757557965863
FPR(2.0) = 0.5786017996637991
F1-Score(0.0) = 0.23851321874182008
F1-Score(1.0) = 0.18051538259268998
F1-Score(2.0) = 0.8099419350163672
Weighted precision: 0.6785988884472671
Weighted recall: 0.6637040138553186
Weighted F1 score: 0.6680457433075503
Weighted false positive rate: 0.4643017153616383
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6530322538047605
Recall = 0.6530322538047605
F1 Score = 0.6530322538047605
Precision(0.0) = 0.337910284463895                                              
Precision(1.0) = 0.15177130561745947
Precision(2.0) = 0.7898646682188591
Recall(0.0) = 0.19998057498057498
Recall(1.0) = 0.22806004618937645
Recall(2.0) = 0.8129446299929608
FPR(0.0) = 0.08022776385740232
FPR(1.0) = 0.13426100495055526
FPR(2.0) = 0.5990914371058745
F1-Score(0.0) = 0.25126098275301006
F1-Score(1.0) = 0.18225441793937158
F1-Score(2.0) = 0.801238476924326
Weighted precision: 0.652245441134469
Weighted recall: 0.6530322538047604
Weighted F1 score: 0.6487811532881358
Weighted false positive rate: 0.46661245971859266
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7496868601552755
Recall = 0.7496868601552755
F1 Score = 0.7496868601552755
Precision(0.0) = 0.3997415000179514                                             
Precision(1.0) = 0.19224121375072017
Precision(2.0) = 0.8136820720569552
Recall(0.0) = 0.21439161997188685
Recall(1.0) = 0.11535912875623038
Recall(2.0) = 0.9181134308173443
FPR(0.0) = 0.050589438520473005
FPR(1.0) = 0.0483854268524164
FPR(2.0) = 0.7176773389349276
F1-Score(0.0) = 0.2790965833604893
F1-Score(1.0) = 0.1441921601815006
F1-Score(2.0) = 0.8627490226540918
Weighted precision: 0.7010647813019608
Weighted recall: 0.7496868601552755
Weighted F1 score: 0.7182700578868461
Weighted false positive rate: 0.5663390644630926
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7262572979616921
Recall = 0.7262572979616921
F1 Score = 0.7262572979616921
Precision(0.0) = 0.3686324087156987                                             
Precision(1.0) = 0.1642261148256617
Precision(2.0) = 0.8177575801998583
Recall(0.0) = 0.17418039987350223
Recall(1.0) = 0.18087760939687178
Recall(2.0) = 0.8903371683181486
FPR(0.0) = 0.0508989754258068
FPR(1.0) = 0.08457800468604086
FPR(2.0) = 0.6646469146803297
F1-Score(0.0) = 0.23657710113110297
F1-Score(1.0) = 0.1721501390176089
F1-Score(2.0) = 0.8525053647727057
Weighted precision: 0.6973036789255004
Weighted recall: 0.726257297961692
Weighted F1 score: 0.7054828349695798
Weighted false positive rate: 0.5263811927538695
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.6672656835877427
Recall = 0.6672656835877427
F1 Score = 0.6672656835877427
Precision(0.0) = 0.2658244391200174                                             
Precision(1.0) = 0.1669755068342354
Precision(2.0) = 0.8394359683440065
Recall(0.0) = 0.15614923998157532
Recall(1.0) = 0.35796884833228443
Recall(2.0) = 0.7910620338787073
FPR(0.0) = 0.06733523782887509
FPR(1.0) = 0.17202459659239447
FPR(2.0) = 0.527487519766829
F1-Score(0.0) = 0.19673399642125963
F1-Score(1.0) = 0.22772710780817976
F1-Score(2.0) = 0.814531417424513
Weighted precision: 0.7028869758589982
Weighted recall: 0.6672656835877427
Weighted F1 score: 0.679541109798276
Weighted false positive rate: 0.43411303777584126
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.6782896320885419
Recall = 0.6782896320885419
F1 Score = 0.6782896320885419
Precision(0.0) = 0.2746374924025354                                             
Precision(1.0) = 0.1532608978868652
Precision(2.0) = 0.831714738246082
Recall(0.0) = 0.18605882352941178
Recall(1.0) = 0.2747956085026863
Recall(2.0) = 0.8064705169138746
FPR(0.0) = 0.07617085101824034
FPR(1.0) = 0.14010709481599007
FPR(2.0) = 0.5829798754625034
F1-Score(0.0) = 0.22183259108601888
F1-Score(1.0) = 0.19677505687140373
F1-Score(2.0) = 0.8188981224992306
Weighted precision: 0.6996323901350983
Weighted recall: 0.6782896320885419
Weighted F1 score: 0.6862085429555465
Weighted false positive rate: 0.4775474533852757
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! 
/lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.6635872277616727
Recall = 0.6635872277616727
F1 Score = 0.6635872277616727
Precision(0.0) = 0.26733981315466643                                            
Precision(1.0) = 0.13935380585067675
Precision(2.0) = 0.8268751610963141
Recall(0.0) = 0.19813959994404812
Recall(1.0) = 0.2771746996671009
Recall(2.0) = 0.791382287640819
FPR(0.0) = 0.0972018779342723
FPR(1.0) = 0.13553126145947927
FPR(2.0) = 0.5700947800254633
F1-Score(0.0) = 0.22759590279172526
F1-Score(1.0) = 0.18546317369618903
F1-Score(2.0) = 0.8087394957983193
Weighted precision: 0.6914826234447389
Weighted recall: 0.6635872277616726
Weighted F1 score: 0.6747795794506197
Weighted false positive rate: 0.46641514718088756



SPORTS
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.7254584172894583
Recall = 0.7254584172894583
F1 Score = 0.7254584172894583
Precision(0.0) = 0.5000699665432711                                             
Precision(1.0) = 0.1634540582591408
Precision(2.0) = 0.7879231502774406
Recall(0.0) = 0.33766836173721826
Recall(1.0) = 0.0795942419395572
Recall(2.0) = 0.901967265008193
FPR(0.0) = 0.08236228591548116
FPR(1.0) = 0.03544743319268636
FPR(2.0) = 0.6362577166142059
F1-Score(0.0) = 0.40312780412767596
F1-Score(1.0) = 0.10705692529793077
F1-Score(2.0) = 0.8410970113375781
Weighted precision: 0.681476348224185
Weighted recall: 0.7254584172894583
Weighted F1 score: 0.6964364996576113
Weighted false positive rate: 0.4795258530118316
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.749107941866129
Recall = 0.749107941866129
F1 Score = 0.749107941866129
Precision(0.0) = 0.25962338582919836                                            
Precision(1.0) = 0.15977961432506887
Precision(2.0) = 0.8257775494878105
Recall(0.0) = 0.20935434166708086
Recall(1.0) = 0.06983744732089103
Recall(2.0) = 0.8976252738709449
FPR(0.0) = 0.07678072603378953
FPR(1.0) = 0.03397088033463483
FPR(2.0) = 0.7641011748602715
F1-Score(0.0) = 0.23179473068721193
F1-Score(1.0) = 0.09719312945119397
F1-Score(2.0) = 0.8602037654445367
Weighted precision: 0.7048741707035274
Weighted recall: 0.749107941866129
Weighted F1 score: 0.7239923937267607
Weighted false positive rate: 0.6239607230948249
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7848654659477218
Recall = 0.7848654659477218
F1 Score = 0.7848654659477218
Precision(0.0) = 0.20802681052803662                                            
Precision(1.0) = 0.14847024964024275
Precision(2.0) = 0.8568501198774937
Recall(0.0) = 0.19981471013127317
Recall(1.0) = 0.04711044053125806
Recall(2.0) = 0.9100300045746885
FPR(0.0) = 0.07511469934738824
FPR(1.0) = 0.02067572083978975
FPR(2.0) = 0.7925649905747227
F1-Score(0.0) = 0.2038380828808048
F1-Score(1.0) = 0.0715254543810471
F1-Score(2.0) = 0.8826397532245724
Weighted precision: 0.7481878314984483
Weighted recall: 0.7848654659477217
Weighted F1 score: 0.7639807559167778
Weighted false positive rate: 0.6732208767096225
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.7442856327198676
Recall = 0.7442856327198676
F1 Score = 0.7442856327198676
Precision(0.0) = 0.4248702529038636                                             
Precision(1.0) = 0.20043731778425655
Precision(2.0) = 0.8131339284709167
Recall(0.0) = 0.2984750716166556
Recall(1.0) = 0.10308634262151693
Recall(2.0) = 0.9051169434924533
FPR(0.0) = 0.0795100590502981
FPR(1.0) = 0.03389882883718056
FPR(2.0) = 0.6565608622565016
F1-Score(0.0) = 0.3506297057973724
F1-Score(1.0) = 0.13614984734714086
F1-Score(2.0) = 0.8566633755251742
Weighted precision: 0.7026300254078424
Weighted recall: 0.7442856327198676
Weighted F1 score: 0.7185833404865359
Weighted false positive rate: 0.5142553828638476
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6914980247158122
Recall = 0.6914980247158122
F1 Score = 0.6914980247158122
Precision(0.0) = 0.3730122671512949                                             
Precision(1.0) = 0.16359126984126984
Precision(2.0) = 0.779878607032654
Recall(0.0) = 0.29237891737891736
Recall(1.0) = 0.09520785219399538
Recall(2.0) = 0.8611556261139152
FPR(0.0) = 0.10062442827029391
FPR(1.0) = 0.05127534574823933
FPR(2.0) = 0.6732907401261201
F1-Score(0.0) = 0.3278099421042124
F1-Score(1.0) = 0.12036496350364964
F1-Score(2.0) = 0.8185043755538395
Weighted precision: 0.6520002262902431
Weighted recall: 0.6914980247158122
Weighted F1 score: 0.6685789616404583
Weighted false positive rate: 0.5166885388604656
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7223606691125133
Recall = 0.7223606691125133
F1 Score = 0.7223606691125133
Precision(0.0) = 0.30433251971460756                                            
Precision(1.0) = 0.15517019082001032
Precision(2.0) = 0.804413855200634
Recall(0.0) = 0.24968709683630833
Recall(1.0) = 0.06934800772134028
Recall(2.0) = 0.8819846166849802
FPR(0.0) = 0.08968966727587417
FPR(1.0) = 0.03768967064318336
FPR(2.0) = 0.7320698968167864
F1-Score(0.0) = 0.27431484752647
F1-Score(1.0) = 0.09585631508731407
F1-Score(2.0) = 0.8414151904940071
Weighted precision: 0.6775750317623902
Weighted recall: 0.7223606691125133
Weighted F1 score: 0.6967332722795344
Weighted false positive rate: 0.5818099038483572
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7644371607087985
Recall = 0.7644371607087985
F1 Score = 0.7644371607087985
Precision(0.0) = 0.45599145683453235                                            
Precision(1.0) = 0.2088282504012841
Precision(2.0) = 0.8166995643490347
Recall(0.0) = 0.28507677711795915
Recall(1.0) = 0.07917959953745968
Recall(2.0) = 0.9300392365498438
FPR(0.0) = 0.05802723005257762
FPR(1.0) = 0.027562643642809612
FPR(2.0) = 0.6992203163288038
F1-Score(0.0) = 0.35082484703033445
F1-Score(1.0) = 0.11482282335289704
F1-Score(2.0) = 0.8696922962115371
Weighted precision: 0.712974656066587
Weighted recall: 0.7644371607087984
Weighted F1 score: 0.7305459833733309
Weighted false positive rate: 0.5492473507329895
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.7696975770917498
Recall = 0.7696975770917498
F1 Score = 0.7696975770917498
Precision(0.0) = 0.4256615812507669                                             
Precision(1.0) = 0.2734724921828784
Precision(2.0) = 0.8261347157629375
Recall(0.0) = 0.2663135267925687
Recall(1.0) = 0.12728130899937068
Recall(2.0) = 0.9298144186853211
FPR(0.0) = 0.05610404139281219
FPR(1.0) = 0.03257192002697593
FPR(2.0) = 0.6821803975070541
F1-Score(0.0) = 0.3276402159711619
F1-Score(1.0) = 0.1737123225165741
F1-Score(2.0) = 0.8749136924564069
Weighted precision: 0.7234934882294725
Weighted recall: 0.7696975770917498
Weighted F1 score: 0.7393963784133513
Weighted false positive rate: 0.540553936018592
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.7691366454969232
Recall = 0.7691366454969232
F1 Score = 0.7691366454969232
Precision(0.0) = 0.4223121800214311                                             
Precision(1.0) = 0.24202318662152458
Precision(2.0) = 0.8326732446601497
Recall(0.0) = 0.3129705882352941
Recall(1.0) = 0.11020789535155337
Recall(2.0) = 0.9187446954694257
FPR(0.0) = 0.06636000164122016
FPR(1.0) = 0.031852516124581794
FPR(2.0) = 0.6595975092500677
F1-Score(0.0) = 0.35951146172947956
F1-Score(1.0) = 0.15145095017976373
F1-Score(2.0) = 0.8735940280870134
Weighted precision: 0.7276989179802211
Weighted recall: 0.7691366454969232
Weighted F1 score: 0.7435904368403109
Weighted false positive rate: 0.5269466725127929
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.743854395633568
Recall = 0.743854395633568
F1 Score = 0.743854395633568
Precision(0.0) = 0.38183250949208397                                            
Precision(1.0) = 0.19259071301700076
Precision(2.0) = 0.8385929490121012
Recall(0.0) = 0.37277940970765144
Recall(1.0) = 0.10985670864090318
Recall(2.0) = 0.8766000603020585
FPR(0.0) = 0.10803129890453834
FPR(1.0) = 0.036464063072973965
FPR(2.0) = 0.5805158674022728
F1-Score(0.0) = 0.37725165445730263
F1-Score(1.0) = 0.1399078341013825
F1-Score(2.0) = 0.8571754032122969
Weighted precision: 0.7218504621767307
Weighted recall: 0.7438543956335679
Weighted F1 score: 0.731687722086218
Weighted false positive rate: 0.46886562501335316
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!


TOYS
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6880471187605718
Recall = 0.6880471187605718
F1 Score = 0.6880471187605718
Precision(0.0) = 0.4110189513168512                                             
Precision(1.0) = 0.15511852044803334
Precision(2.0) = 0.8161391430297985
Recall(0.0) = 0.48568066245189667
Recall(1.0) = 0.10026096472767068
Recall(2.0) = 0.8078890771637122
FPR(0.0) = 0.1698047565954379
FPR(1.0) = 0.047519631973745896
FPR(2.0) = 0.4769904594588
F1-Score(0.0) = 0.44524153571752
F1-Score(1.0) = 0.12179782175180243
F1-Score(2.0) = 0.8119931549230864
Weighted precision: 0.6837666808504048
Weighted recall: 0.6880471187605718
Weighted F1 score: 0.6848104451354275
Weighted false positive rate: 0.3823619667885555
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7400967387487398
Recall = 0.7400967387487398
F1 Score = 0.7400967387487398
Precision(0.0) = 0.2645938222887468                                             
Precision(1.0) = 0.16913222510294343
Precision(2.0) = 0.8362565391946145
Recall(0.0) = 0.2899497986977484
Recall(1.0) = 0.07418556425178942
Recall(2.0) = 0.8744610926567249
FPR(0.0) = 0.10364103580309258
FPR(1.0) = 0.03371099381841358
FPR(2.0) = 0.6908435040492757
F1-Score(0.0) = 0.276692121614571
F1-Score(1.0) = 0.1031340091137357
F1-Score(2.0) = 0.8549322148671245
Weighted precision: 0.7146300845860125
Weighted recall: 0.7400967387487398
Weighted F1 score: 0.7253870013171548
Weighted false positive rate: 0.5682922724195217
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7630402847179985
Recall = 0.7630402847179985
F1 Score = 0.7630402847179985
Precision(0.0) = 0.2063833457933176                                             
Precision(1.0) = 0.15516048101046803
Precision(2.0) = 0.8673751353229708
Recall(0.0) = 0.28176622071477925
Recall(1.0) = 0.07121160985487682
Recall(2.0) = 0.8731987163962218
FPR(0.0) = 0.10698708576053537
FPR(1.0) = 0.029670646856865067
FPR(2.0) = 0.6960238481434395
F1-Score(0.0) = 0.23825425382894397
F1-Score(1.0) = 0.09762005198056851
F1-Score(2.0) = 0.8702771836425445
Weighted precision: 0.7573466924849049
Weighted recall: 0.7630402847179985
Weighted F1 score: 0.7585557649617435
Weighted false positive rate: 0.5957218654788384
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.7036998268085187
Recall = 0.7036998268085187
F1 Score = 0.7036998268085187
Precision(0.0) = 0.35904267227869074                                            
Precision(1.0) = 0.18213876399541568
Precision(2.0) = 0.8419335378787387
Recall(0.0) = 0.46404699210046585
Recall(1.0) = 0.12907659627639634
Recall(2.0) = 0.8132162123215148
FPR(0.0) = 0.16302323859850923
FPR(1.0) = 0.04777870481958736
FPR(2.0) = 0.4819143676456047
F1-Score(0.0) = 0.404846954875355
F1-Score(1.0) = 0.15108413470327983
F1-Score(2.0) = 0.8273257481594798
Weighted precision: 0.7122830583902792
Weighted recall: 0.7036998268085188
Weighted F1 score: 0.7063564093223084
Weighted false positive rate: 0.39641613787222
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.7098313030273018
Recall = 0.7098313030273018
F1 Score = 0.7098313030273018
Precision(0.0) = 0.40217913795866045                                            
Precision(1.0) = 0.1702127659574468
Precision(2.0) = 0.7853733651525857
Recall(0.0) = 0.325045325045325
Recall(1.0) = 0.06651270207852195
Recall(2.0) = 0.8822732106216957
FPR(0.0) = 0.09892746821514271
FPR(1.0) = 0.03415518227044385
FPR(2.0) = 0.6678767009624959
F1-Score(0.0) = 0.35952159278092094
F1-Score(1.0) = 0.09564928595151112
F1-Score(2.0) = 0.8310080690666967
Weighted precision: 0.6616254704664536
Weighted recall: 0.7098313030273019
Weighted F1 score: 0.6808001503060633
Weighted false positive rate: 0.5107906544753843
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7088283209166957
Recall = 0.7088283209166957
F1 Score = 0.7088283209166957
Precision(0.0) = 0.2969487016903543                                             
Precision(1.0) = 0.1747545182866088
Precision(2.0) = 0.8212359483967837
Recall(0.0) = 0.3697263782180887
Recall(1.0) = 0.07075974531101444
Recall(2.0) = 0.8432457104217733
FPR(0.0) = 0.13755582721099963
FPR(1.0) = 0.03335557421744682
FPR(2.0) = 0.6266129590729669
F1-Score(0.0) = 0.32936514743468787
F1-Score(1.0) = 0.10073211246231774
F1-Score(2.0) = 0.8320953097449943
Weighted precision: 0.6913606197871794
Weighted recall: 0.7088283209166957
Weighted F1 score: 0.6974434225806017
Weighted false positive rate: 0.5063526814181091
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7800215097818294
Recall = 0.7800215097818294
F1 Score = 0.7800215097818294
Precision(0.0) = 0.4966485660953674                                             
Precision(1.0) = 0.23275862068965517
Precision(2.0) = 0.8398462949110826
Recall(0.0) = 0.41136371622333884
Recall(1.0) = 0.08380500273872558
Recall(2.0) = 0.9258695218461129
FPR(0.0) = 0.0711326670703413
FPR(1.0) = 0.025381789307103435
FPR(2.0) = 0.5914234796168412
F1-Score(0.0) = 0.45000096096557823
F1-Score(1.0) = 0.12323801852597666
F1-Score(2.0) = 0.8807624421936978
Weighted precision: 0.7387394540860354
Weighted recall: 0.7800215097818294
Weighted F1 score: 0.7542340964006251
Weighted false positive rate: 0.46795944577611526
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.722041173197679
Recall = 0.722041173197679
F1 Score = 0.722041173197679
Precision(0.0) = 0.3073264941645554                                             
Precision(1.0) = 0.2169811320754717
Precision(2.0) = 0.8349786221414469
Recall(0.0) = 0.3787041302011362
Recall(1.0) = 0.10041692888609188
Recall(2.0) = 0.8519930090144578
FPR(0.0) = 0.13326807439518948
FPR(1.0) = 0.03490579262632654
FPR(2.0) = 0.5870050541068494
F1-Score(0.0) = 0.33930209097578873
F1-Score(1.0) = 0.1372949717666039
F1-Score(2.0) = 0.8434000140874833
Weighted precision: 0.7094215950007333
Weighted recall: 0.722041173197679
Weighted F1 score: 0.7132826416683253
Weighted false positive rate: 0.47722009432604445
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.7228053001985404
Recall = 0.7228053001985404
F1 Score = 0.7228053001985404
Precision(0.0) = 0.3250575009135659                                             
Precision(1.0) = 0.21168406790467842
Precision(2.0) = 0.8510559447398356
Recall(0.0) = 0.44476470588235295
Recall(1.0) = 0.12408315814062135
Recall(2.0) = 0.8353069555025664
FPR(0.0) = 0.14314631021796315
FPR(1.0) = 0.04264391404821854
FPR(2.0) = 0.5222813825467015
F1-Score(0.0) = 0.3756038797332373
F1-Score(1.0) = 0.15645617342130066
F1-Score(2.0) = 0.8431079100006375
Weighted precision: 0.7264464056702133
Weighted recall: 0.7228053001985403
Weighted F1 score: 0.7223538614329609
Weighted false positive rate: 0.43087690701142356
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.6685992800484215
Recall = 0.6685992800484215
F1 Score = 0.6685992800484215
Precision(0.0) = 0.30031785896480007                                            
Precision(1.0) = 0.16709777547853077
Precision(2.0) = 0.8640664005978598
Recall(0.0) = 0.5352496852706672
Recall(1.0) = 0.14025184541901867
Recall(2.0) = 0.7447578324150974
FPR(0.0) = 0.22322378716744914
FPR(1.0) = 0.05534928492849285
FPR(2.0) = 0.40312161078889047
F1-Score(0.0) = 0.38475654206782134
F1-Score(1.0) = 0.15250236071765813
F1-Score(2.0) = 0.7999882229108547
Weighted precision: 0.7273410878307298
Weighted recall: 0.6685992800484215
Weighted F1 score: 0.6894420749216594
Weighted false positive rate: 0.350293962933254
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!


MOVIES
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6420941970874244
Recall = 0.6420941970874244
F1 Score = 0.6420941970874244
Precision(0.0) = 0.3420868401810856                                             
Precision(1.0) = 0.12622935791830908
Precision(2.0) = 0.7716438077911526
Recall(0.0) = 0.1888829714128642
Recall(1.0) = 0.20285798467884503
Recall(2.0) = 0.8134775808133472
FPR(0.0) = 0.08863078122511255
FPR(1.0) = 0.12219072315986873
FPR(2.0) = 0.6309201376180368
F1-Score(0.0) = 0.243382495365118
F1-Score(1.0) = 0.1556221090275031
F1-Score(2.0) = 0.792008665739058
Weighted precision: 0.635727854429002
Weighted recall: 0.6420941970874244
Weighted F1 score: 0.6334623120535939
Weighted false positive rate: 0.4838358390904425
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7120946091369408
Recall = 0.7120946091369408
F1 Score = 0.7120946091369408
Precision(0.0) = 0.2819664998912334                                             
Precision(1.0) = 0.1584804079543516
Precision(2.0) = 0.853021126252794
Recall(0.0) = 0.16106665341219742
Recall(1.0) = 0.27961736571008095
Recall(2.0) = 0.8361403632765566
FPR(0.0) = 0.052748994815870726
FPR(1.0) = 0.13734074216163702
FPR(2.0) = 0.5812849321318581
F1-Score(0.0) = 0.2050203248817677
F1-Score(1.0) = 0.20230129826132198
F1-Score(2.0) = 0.8444963951745306
Weighted precision: 0.7291426431163083
Weighted recall: 0.7120946091369408
Weighted F1 score: 0.717253259423244
Weighted false positive rate: 0.4834692782463067
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7752511532800569
Recall = 0.7752511532800569
F1 Score = 0.7752511532800569
Precision(0.0) = 0.24504214874488328                                            
Precision(1.0) = 0.15637934137124349
Precision(2.0) = 0.8732790518197308
Recall(0.0) = 0.20586018466176748
Recall(1.0) = 0.1552679120922753
Recall(2.0) = 0.8887610667097225
FPR(0.0) = 0.06262685150872863
FPR(1.0) = 0.0640962537599125
FPR(2.0) = 0.6723159879005742
F1-Score(0.0) = 0.2237487733071639
F1-Score(1.0) = 0.1558216448836468
F1-Score(2.0) = 0.8809520435644786
Weighted precision: 0.7658612359883328
Weighted recall: 0.7752511532800569
Weighted F1 score: 0.7703459927777941
Weighted false positive rate: 0.5742902464492723
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.6637040138553185
Recall = 0.6637040138553185
F1 Score = 0.6637040138553185
Precision(0.0) = 0.3004484304932735                                             
Precision(1.0) = 0.13901451231859602
Precision(2.0) = 0.8145897234403914
Recall(0.0) = 0.1977487774530513
Recall(1.0) = 0.2573409971260777
Recall(2.0) = 0.8053468832820616
FPR(0.0) = 0.09060832626286208
FPR(1.0) = 0.13138757557965863
FPR(2.0) = 0.5786017996637991
F1-Score(0.0) = 0.23851321874182008
F1-Score(1.0) = 0.18051538259268998
F1-Score(2.0) = 0.8099419350163672
Weighted precision: 0.6785988884472671
Weighted recall: 0.6637040138553186
Weighted F1 score: 0.6680457433075503
Weighted false positive rate: 0.4643017153616383
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6530322538047605
Recall = 0.6530322538047605
F1 Score = 0.6530322538047605
Precision(0.0) = 0.337910284463895                                              
Precision(1.0) = 0.15177130561745947
Precision(2.0) = 0.7898646682188591
Recall(0.0) = 0.19998057498057498
Recall(1.0) = 0.22806004618937645
Recall(2.0) = 0.8129446299929608
FPR(0.0) = 0.08022776385740232
FPR(1.0) = 0.13426100495055526
FPR(2.0) = 0.5990914371058745
F1-Score(0.0) = 0.25126098275301006
F1-Score(1.0) = 0.18225441793937158
F1-Score(2.0) = 0.801238476924326
Weighted precision: 0.652245441134469
Weighted recall: 0.6530322538047604
Weighted F1 score: 0.6487811532881358
Weighted false positive rate: 0.46661245971859266
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7496868601552755
Recall = 0.7496868601552755
F1 Score = 0.7496868601552755
Precision(0.0) = 0.3997415000179514                                             
Precision(1.0) = 0.19224121375072017
Precision(2.0) = 0.8136820720569552
Recall(0.0) = 0.21439161997188685
Recall(1.0) = 0.11535912875623038
Recall(2.0) = 0.9181134308173443
FPR(0.0) = 0.050589438520473005
FPR(1.0) = 0.0483854268524164
FPR(2.0) = 0.7176773389349276
F1-Score(0.0) = 0.2790965833604893
F1-Score(1.0) = 0.1441921601815006
F1-Score(2.0) = 0.8627490226540918
Weighted precision: 0.7010647813019608
Weighted recall: 0.7496868601552755
Weighted F1 score: 0.7182700578868461
Weighted false positive rate: 0.5663390644630926
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7262572979616921
Recall = 0.7262572979616921
F1 Score = 0.7262572979616921
Precision(0.0) = 0.3686324087156987                                             
Precision(1.0) = 0.1642261148256617
Precision(2.0) = 0.8177575801998583
Recall(0.0) = 0.17418039987350223
Recall(1.0) = 0.18087760939687178
Recall(2.0) = 0.8903371683181486
FPR(0.0) = 0.0508989754258068
FPR(1.0) = 0.08457800468604086
FPR(2.0) = 0.6646469146803297
F1-Score(0.0) = 0.23657710113110297
F1-Score(1.0) = 0.1721501390176089
F1-Score(2.0) = 0.8525053647727057
Weighted precision: 0.6973036789255004
Weighted recall: 0.726257297961692
Weighted F1 score: 0.7054828349695798
Weighted false positive rate: 0.5263811927538695
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.6672656835877427
Recall = 0.6672656835877427
F1 Score = 0.6672656835877427
Precision(0.0) = 0.2658244391200174                                             
Precision(1.0) = 0.1669755068342354
Precision(2.0) = 0.8394359683440065
Recall(0.0) = 0.15614923998157532
Recall(1.0) = 0.35796884833228443
Recall(2.0) = 0.7910620338787073
FPR(0.0) = 0.06733523782887509
FPR(1.0) = 0.17202459659239447
FPR(2.0) = 0.527487519766829
F1-Score(0.0) = 0.19673399642125963
F1-Score(1.0) = 0.22772710780817976
F1-Score(2.0) = 0.814531417424513
Weighted precision: 0.7028869758589982
Weighted recall: 0.6672656835877427
Weighted F1 score: 0.679541109798276
Weighted false positive rate: 0.43411303777584126
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.6782896320885419
Recall = 0.6782896320885419
F1 Score = 0.6782896320885419
Precision(0.0) = 0.2746374924025354                                             
Precision(1.0) = 0.1532608978868652
Precision(2.0) = 0.831714738246082
Recall(0.0) = 0.18605882352941178
Recall(1.0) = 0.2747956085026863
Recall(2.0) = 0.8064705169138746
FPR(0.0) = 0.07617085101824034
FPR(1.0) = 0.14010709481599007
FPR(2.0) = 0.5829798754625034
F1-Score(0.0) = 0.22183259108601888
F1-Score(1.0) = 0.19677505687140373
F1-Score(2.0) = 0.8188981224992306
Weighted precision: 0.6996323901350983
Weighted recall: 0.6782896320885419
Weighted F1 score: 0.6862085429555465
Weighted false positive rate: 0.4775474533852757
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.6635872277616727
Recall = 0.6635872277616727
F1 Score = 0.6635872277616727
Precision(0.0) = 0.26733981315466643                                            
Precision(1.0) = 0.13935380585067675
Precision(2.0) = 0.8268751610963141
Recall(0.0) = 0.19813959994404812
Recall(1.0) = 0.2771746996671009
Recall(2.0) = 0.791382287640819
FPR(0.0) = 0.0972018779342723
FPR(1.0) = 0.13553126145947927
FPR(2.0) = 0.5700947800254633
F1-Score(0.0) = 0.22759590279172526
F1-Score(1.0) = 0.18546317369618903
F1-Score(2.0) = 0.8087394957983193
Weighted precision: 0.6914826234447389
Weighted recall: 0.6635872277616726
Weighted F1 score: 0.6747795794506197
Weighted false positive rate: 0.46641514718088756
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!


VIDEO GAMES

!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6616893881704417
Recall = 0.6616893881704417
F1 Score = 0.6616893881704417
Precision(0.0) = 0.39253494687346224                                            
Precision(1.0) = 0.131167315944551
Precision(2.0) = 0.7917840911976033
Recall(0.0) = 0.37001786695986805
Recall(1.0) = 0.13959508376125937
Recall(2.0) = 0.7984647326083718
FPR(0.0) = 0.13970927259466664
FPR(1.0) = 0.08046179090482888
FPR(2.0) = 0.5502952443696166
F1-Score(0.0) = 0.3809439585415248
F1-Score(1.0) = 0.13525003823214557
F1-Score(2.0) = 0.7951103792028871
Weighted precision: 0.6605954492338669
Weighted recall: 0.6616893881704417
Weighted F1 score: 0.6610565585714491
Weighted false positive rate: 0.4321556960395538
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.6821582709364628
Recall = 0.6821582709364628
F1 Score = 0.6821582709364628
Precision(0.0) = 0.22869667707450217                                            
Precision(1.0) = 0.14222904417503512
Precision(2.0) = 0.8424321391424505
Recall(0.0) = 0.27486455589243997
Recall(1.0) = 0.1828550404709345
Recall(2.0) = 0.7928263481518129
FPR(0.0) = 0.1192189927064223
FPR(1.0) = 0.10200855150393852
FPR(2.0) = 0.5983089996578077
F1-Score(0.0) = 0.24966421742909062
F1-Score(1.0) = 0.16000351205806604
F1-Score(2.0) = 0.8168768444029368
Weighted precision: 0.713210694472637
Weighted recall: 0.6821582709364629
Weighted F1 score: 0.6966254239784287
Weighted false positive rate: 0.5016948148046314
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7537618309105868
Recall = 0.7537618309105868
F1 Score = 0.7537618309105868
Precision(0.0) = 0.21131485391997007                                            
Precision(1.0) = 0.12938967136150234
Precision(2.0) = 0.8674022215494013
Recall(0.0) = 0.2482727215627159
Recall(1.0) = 0.10942804391415696
Recall(2.0) = 0.8624902451494847
FPR(0.0) = 0.09149744087498662
FPR(1.0) = 0.05634247865585027
FPR(2.0) = 0.6873262899478322
F1-Score(0.0) = 0.22830779894011813
F1-Score(1.0) = 0.11857460928676683
F1-Score(2.0) = 0.8649392596465633
Weighted precision: 0.7559807651276141
Weighted recall: 0.7537618309105868
Weighted F1 score: 0.7546726021804031
Weighted false positive rate: 0.5889280403892558
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.6707078012294692
Recall = 0.6707078012294692
F1 Score = 0.6707078012294692
Precision(0.0) = 0.33816583966042923                                            
Precision(1.0) = 0.12411668780576192
Precision(2.0) = 0.8206761423158003
Recall(0.0) = 0.3273532220261003
Recall(1.0) = 0.17118580532300387
Recall(2.0) = 0.795146829399713
FPR(0.0) = 0.12607836549685958
FPR(1.0) = 0.09958489127859667
FPR(2.0) = 0.5484228221101553
F1-Score(0.0) = 0.3326716951171099
F1-Score(1.0) = 0.14390000525182503
F1-Score(2.0) = 0.8077098097368647
Weighted precision: 0.6882883638374367
Weighted recall: 0.6707078012294692
Weighted F1 score: 0.6790448023441975
Weighted false positive rate: 0.4447938801150807
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.7152179415227845
Recall = 0.7152179415227845
F1 Score = 0.7152179415227845
Precision(0.0) = 0.4154163326079487                                             
Precision(1.0) = 0.18324456599971212
Precision(2.0) = 0.7719798902991668
Recall(0.0) = 0.23484848484848486
Recall(1.0) = 0.07349884526558892
Recall(2.0) = 0.9095613233686292
FPR(0.0) = 0.06766628219915417
FPR(1.0) = 0.03450792453748191
FPR(2.0) = 0.7441918353800199
F1-Score(0.0) = 0.3000620475698035
F1-Score(1.0) = 0.10491614126179587
F1-Score(2.0) = 0.8351422432316288
Weighted precision: 0.6552761885019723
Weighted recall: 0.7152179415227846
Weighted F1 score: 0.6746156117254611
Weighted false positive rate: 0.5615839836394405
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.6720072590915153
Recall = 0.6720072590915153
F1 Score = 0.6720072590915153
Precision(0.0) = 0.2846933088548667                                             
Precision(1.0) = 0.15491568878808795
Precision(2.0) = 0.8308260369525043
Recall(0.0) = 0.3344309013536672
Recall(1.0) = 0.18104814313290502
Recall(2.0) = 0.7888935846504944
FPR(0.0) = 0.13204270100821824
FPR(1.0) = 0.09858847078583179
FPR(2.0) = 0.548371459569262
F1-Score(0.0) = 0.3075642603529339
F1-Score(1.0) = 0.16696557862713057
F1-Score(2.0) = 0.8093170222433413
Weighted precision: 0.6953130151916168
Weighted recall: 0.6720072590915154
Weighted F1 score: 0.6828767686988347
Weighted false positive rate: 0.4510098904548274
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7456724367509987
Recall = 0.7456724367509987
F1 Score = 0.7456724367509987
Precision(0.0) = 0.4087464477423429                                             
Precision(1.0) = 0.16971358927483243
Precision(2.0) = 0.8182222435882027
Recall(0.0) = 0.272918936013212
Recall(1.0) = 0.10169800985941209
Recall(2.0) = 0.9055130677661768
FPR(0.0) = 0.06735571129669486
FPR(1.0) = 0.04571406203691795
FPR(2.0) = 0.6738694586767654
F1-Score(0.0) = 0.3273003097279872
F1-Score(1.0) = 0.12718346843246947
F1-Score(2.0) = 0.8596574300307466
Weighted precision: 0.7039698756019264
Weighted recall: 0.7456724367509987
Weighted F1 score: 0.7204295751207931
Weighted false positive rate: 0.5326116687613768
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.6692355276935891
Recall = 0.6692355276935891
F1 Score = 0.6692355276935891
Precision(0.0) = 0.25354852154583557                                            
Precision(1.0) = 0.17334865020103388
Precision(2.0) = 0.8358693389352562
Recall(0.0) = 0.2802088131429449
Recall(1.0) = 0.23741346758967904
Recall(2.0) = 0.7856675902001681
FPR(0.0) = 0.1288011666699962
FPR(1.0) = 0.10905550146056475
FPR(2.0) = 0.5378127809990388
F1-Score(0.0) = 0.266212848720598
F1-Score(1.0) = 0.2003851005909302
F1-Score(2.0) = 0.8099913575124308
Weighted precision: 0.6990174992310692
Weighted recall: 0.6692355276935891
Weighted F1 score: 0.6829937591928824
Weighted false positive rate: 0.4449049768231888
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.6876048454898184
Recall = 0.6876048454898184
F1 Score = 0.6876048454898184
Precision(0.0) = 0.28703654870523704                                            
Precision(1.0) = 0.16327097978474125
Precision(2.0) = 0.8368445397586308
Recall(0.0) = 0.3201470588235294
Recall(1.0) = 0.19205793039009578
Recall(2.0) = 0.8043082892131108
FPR(0.0) = 0.12326019266101054
FPR(1.0) = 0.09083226985824164
FPR(2.0) = 0.5602382456456998
F1-Score(0.0) = 0.3026890242206835
F1-Score(1.0) = 0.176498368538554
F1-Score(2.0) = 0.8202538949798038
Weighted precision: 0.7061500679152192
Weighted recall: 0.6876048454898185
Weighted F1 score: 0.6964057935494251
Weighted false positive rate: 0.4619355536547704
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.6400029732513566
Recall = 0.6400029732513566
F1 Score = 0.6400029732513566
Precision(0.0) = 0.26318540340207164                                            
Precision(1.0) = 0.13056049822064056
Precision(2.0) = 0.8350822483823186
Recall(0.0) = 0.3873968387187019
Recall(1.0) = 0.1699232884643219
Recall(2.0) = 0.734013101992709
FPR(0.0) = 0.19414084507042254
FPR(1.0) = 0.08959020902090209
FPR(2.0) = 0.49875041259961334
F1-Score(0.0) = 0.3134336803983703
F1-Score(1.0) = 0.14766366895163827
F1-Score(2.0) = 0.7812926236861877
Weighted precision: 0.6965656686684452
Weighted recall: 0.6400029732513565
Weighted F1 score: 0.6637728502968913
Weighted false positive rate: 0.4224844399422945
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!





Books

!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6502331677797171
Recall = 0.6502331677797171
F1 Score = 0.6502331677797171
Precision(0.0) = 0.3476720647773279                                             
Precision(1.0) = 0.1281649600081512
Precision(2.0) = 0.7668036626916525
Recall(0.0) = 0.13572876580538756
Recall(1.0) = 0.21178129472177792
Recall(2.0) = 0.8381382206167138
FPR(0.0) = 0.06213376143251151
FPR(1.0) = 0.12536077414439756
FPR(2.0) = 0.668014786618842
F1-Score(0.0) = 0.19523797756140956
F1-Score(1.0) = 0.1596896026405992
F1-Score(2.0) = 0.8008856446389808
Weighted precision: 0.6334748545100524
Weighted recall: 0.6502331677797171
Weighted F1 score: 0.630770627653285
Weighted false positive rate: 0.5057424899754681
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7790046330384349
Recall = 0.7790046330384349
F1 Score = 0.7790046330384349
Precision(0.0) = 0.35231984977701275                                            
Precision(1.0) = 0.17898118402937127
Precision(2.0) = 0.8239336536627682
Recall(0.0) = 0.11190914061335057
Recall(1.0) = 0.09131045554886615
Recall(2.0) = 0.9465191886352392
FPR(0.0) = 0.026457596890800888
FPR(1.0) = 0.038744748126651365
FPR(2.0) = 0.8160716322573286
F1-Score(0.0) = 0.1698636337916596
F1-Score(1.0) = 0.1209275542069943
F1-Score(2.0) = 0.880982531386602
Weighted precision: 0.7155851642772566
Weighted recall: 0.779004633038435
Weighted F1 score: 0.7355965225137635
Weighted false positive rate: 0.6602786103132159
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7405532639695412
Recall = 0.7405532639695412
F1 Score = 0.7405532639695412
Precision(0.0) = 0.19577354465610053                                            
Precision(1.0) = 0.1406496974982286
Precision(2.0) = 0.8739134969751756
Recall(0.0) = 0.1844576345706928
Recall(1.0) = 0.2049194973298128
Recall(2.0) = 0.8454932590619197
FPR(0.0) = 0.07482165201171569
FPR(1.0) = 0.09580712788259958
FPR(2.0) = 0.6359212660558502
F1-Score(0.0) = 0.18994720544600485
F1-Score(1.0) = 0.1668080705241639
F1-Score(2.0) = 0.8594684976098805
Weighted precision: 0.7608477468641287
Weighted recall: 0.7405532639695414
Weighted F1 score: 0.7500634725081013
Weighted false positive rate: 0.5471033099197067
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.6749709761528653
Recall = 0.6749709761528653
F1 Score = 0.6749709761528653
Precision(0.0) = 0.29632016875659206                                            
Precision(1.0) = 0.1385155290401825
Precision(2.0) = 0.807090656152991
Recall(0.0) = 0.14632946555166526
Recall(1.0) = 0.24659502686492565
Recall(2.0) = 0.8323945691605005
FPR(0.0) = 0.06838332014144739
FPR(1.0) = 0.1264279018983756
FPR(2.0) = 0.6280035597745476
F1-Score(0.0) = 0.19591283292978207
F1-Score(1.0) = 0.17738927215118763
F1-Score(2.0) = 0.819547341603489
Weighted precision: 0.6721871925208243
Weighted recall: 0.6749709761528653
Weighted F1 score: 0.6680972576488795
Weighted false positive rate: 0.4977857579672359
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6531533018608388
Recall = 0.6531533018608388
F1 Score = 0.6531533018608388
Precision(0.0) = 0.30374646701545494                                            
Precision(1.0) = 0.15261463863227856
Precision(2.0) = 0.7791124268736632
Recall(0.0) = 0.16352628852628853
Recall(1.0) = 0.21079676674364897
Recall(2.0) = 0.8237804969372013
FPR(0.0) = 0.07674766999429927
FPR(1.0) = 0.12328950409302665
FPR(2.0) = 0.6469465648854962
F1-Score(0.0) = 0.21259759664962014
F1-Score(1.0) = 0.1770482263656863
F1-Score(2.0) = 0.8008240758266237
Weighted precision: 0.6386194011100088
Weighted recall: 0.6531533018608388
Weighted F1 score: 0.6414096336849384
Weighted false positive rate: 0.500137040833661
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7117099919721143
Recall = 0.7117099919721143
F1 Score = 0.7117099919721143
Precision(0.0) = 0.3313329636998141                                             
Precision(1.0) = 0.16640104317589105
Precision(2.0) = 0.8220555254814013
Recall(0.0) = 0.19561743015038607
Recall(1.0) = 0.19853640266213374
Recall(2.0) = 0.8625475445862565
FPR(0.0) = 0.062036286174217206
FPR(1.0) = 0.09928158109678235
FPR(2.0) = 0.6373814085547425
F1-Score(0.0) = 0.24599849868029153
F1-Score(1.0) = 0.18105384847808095
F1-Score(2.0) = 0.8418148911352391
Weighted precision: 0.6959057825898847
Weighted recall: 0.7117099919721142
Weighted F1 score: 0.7009297115042341
Weighted false positive rate: 0.5104092677978562
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7280600225340571
Recall = 0.7280600225340571
F1 Score = 0.7280600225340571
Precision(0.0) = 0.34018284719198955                                            
Precision(1.0) = 0.1628419313383514
Precision(2.0) = 0.809829544775852
Recall(0.0) = 0.1372852173301943
Recall(1.0) = 0.16194997261274421
Recall(2.0) = 0.9017290682981978
FPR(0.0) = 0.045431382305861474
FPR(1.0) = 0.07649765977553977
FPR(2.0) = 0.7093116507017153
F1-Score(0.0) = 0.1956238734227919
F1-Score(1.0) = 0.1623947272061516
F1-Score(2.0) = 0.8533121043158676
Weighted precision: 0.6869353071289673
Weighted recall: 0.7280600225340572
Weighted F1 score: 0.6993142922382491
Weighted false positive rate: 0.5593007153171738
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.6830313481682178
Recall = 0.6830313481682178
F1 Score = 0.6830313481682178
Precision(0.0) = 0.2549359196397645                                             
Precision(1.0) = 0.16453096396838862
Precision(2.0) = 0.8251114280620432
Recall(0.0) = 0.1318388863299043
Recall(1.0) = 0.28988357457520453
Recall(2.0) = 0.823273044236217
FPR(0.0) = 0.06015941826317998
FPR(1.0) = 0.14179033791898885
FPR(2.0) = 0.6083222225667421
F1-Score(0.0) = 0.1737986405114106
F1-Score(1.0) = 0.20991768492409352
F1-Score(2.0) = 0.8241912110074997
Weighted precision: 0.6900702644120849
Weighted recall: 0.6830313481682178
Weighted F1 score: 0.682385482573005
Weighted false positive rate: 0.4933033269171287
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.6948438714974206
Recall = 0.6948438714974206
F1 Score = 0.6948438714974206
Precision(0.0) = 0.2618230563002681                                             
Precision(1.0) = 0.15032139577594122
Precision(2.0) = 0.8228719639259711
Recall(0.0) = 0.14361764705882352
Recall(1.0) = 0.2294323756131745
Recall(2.0) = 0.8398536959948268
FPR(0.0) = 0.06276299413263794
FPR(1.0) = 0.11967975028455144
FPR(2.0) = 0.6458803357097734
F1-Score(0.0) = 0.18548907882241214
F1-Score(1.0) = 0.1816366158113731
F1-Score(2.0) = 0.8312761111375017
Weighted precision: 0.6907553667792473
Weighted recall: 0.6948438714974204
Weighted F1 score: 0.6897231841625824
Weighted false positive rate: 0.5231669516243833
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.6740254637741179
Recall = 0.6740254637741179
F1 Score = 0.6740254637741179
Precision(0.0) = 0.25327268693144                                               
Precision(1.0) = 0.13685723411050782
Precision(2.0) = 0.8188614304398706
Recall(0.0) = 0.15967268149391523
Recall(1.0) = 0.24808221160804747
Recall(2.0) = 0.8151467806923772
FPR(0.0) = 0.08426917057902973
FPR(1.0) = 0.12387697103043638
FPR(2.0) = 0.620408355731598
F1-Score(0.0) = 0.19586479066575155
F1-Score(1.0) = 0.17640096742654246
F1-Score(2.0) = 0.8169998832425602
Weighted precision: 0.6829545903994862
Weighted recall: 0.6740254637741178
Weighted F1 score: 0.6756973075251458
Weighted false positive rate: 0.502579961115182
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!






MUSIC




ELECTRONICS
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.7429561091979971
Recall = 0.7429561091979971
F1 Score = 0.7429561091979971
Precision(0.0) = 0.518854032315395                                              
Precision(1.0) = 0.17959103032697818
Precision(2.0) = 0.8002160940586506
Recall(0.0) = 0.43885720175920834
Recall(1.0) = 0.03826079636333025
Recall(2.0) = 0.9032939818263072
FPR(0.0) = 0.09929204355881194
FPR(1.0) = 0.015209285630567277
FPR(2.0) = 0.5910377473586609
F1-Score(0.0) = 0.47551458235411825
F1-Score(1.0) = 0.06308228803414355
F1-Score(2.0) = 0.8486364620393918
Weighted precision: 0.6953501212095947
Weighted recall: 0.7429561091979973
Weighted F1 score: 0.7125706816391753
Weighted false positive rate: 0.4484951857460373
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7161612614551592
Recall = 0.7161612614551592
F1 Score = 0.7161612614551592
Precision(0.0) = 0.22719777199604235                                            
Precision(1.0) = 0.1463456430468683
Precision(2.0) = 0.8323717959890821
Recall(0.0) = 0.3081664098613251
Recall(1.0) = 0.057127567061341894
Recall(2.0) = 0.8438052159163192
FPR(0.0) = 0.13480653801162115
FPR(1.0) = 0.03082439715609898
FPR(2.0) = 0.685625071290065
F1-Score(0.0) = 0.2615592305096186
F1-Score(1.0) = 0.08217662200197262
F1-Score(2.0) = 0.8380495115355525
Weighted precision: 0.7053262860204083
Weighted recall: 0.7161612614551592
Weighted F1 score: 0.7083586915806468
Weighted false positive rate: 0.5674172679129442
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7578076601221228
Recall = 0.7578076601221228
F1 Score = 0.7578076601221228
Precision(0.0) = 0.18989081225033289                                            
Precision(1.0) = 0.12600361663652804
Precision(2.0) = 0.8610605876548223
Recall(0.0) = 0.27991332202751085
Recall(1.0) = 0.0345833912370213
Recall(2.0) = 0.8702638518877318
FPR(0.0) = 0.11791511550561519
FPR(1.0) = 0.01835596876614104
FPR(2.0) = 0.7320415588970234
F1-Score(0.0) = 0.22627714062668589
F1-Score(1.0) = 0.05427129416163001
F1-Score(2.0) = 0.86563775870823
Weighted precision: 0.7484937783224306
Weighted recall: 0.7578076601221228
Weighted F1 score: 0.7505053671143231
Weighted false positive rate: 0.6261203032909024
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.732243115162819
Recall = 0.732243115162819
F1 Score = 0.732243115162819
Precision(0.0) = 0.38480056068501084                                            
Precision(1.0) = 0.1783717679944095
Precision(2.0) = 0.817148417243971
Recall(0.0) = 0.36540409155357506
Recall(1.0) = 0.06378857928276896
Recall(2.0) = 0.8787083273290018
FPR(0.0) = 0.11496301526652355
FPR(1.0) = 0.024221542391561858
FPR(2.0) = 0.6206466923761496
F1-Score(0.0) = 0.3748515791973403
F1-Score(1.0) = 0.09397146801656694
F1-Score(2.0) = 0.8468110542872496
Weighted precision: 0.6974094956811103
Weighted recall: 0.7322431151628191
Weighted F1 score: 0.7118720618549524
Weighted false positive rate: 0.49207436519705394
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6959602962376064
Recall = 0.6959602962376064
F1 Score = 0.6959602962376064
Precision(0.0) = 0.37453418197407906                                            
Precision(1.0) = 0.15734888996921081
Precision(2.0) = 0.7859444276154545
Recall(0.0) = 0.3676832426832427
Recall(1.0) = 0.056062355658198615
Recall(2.0) = 0.8548877473078824
FPR(0.0) = 0.12572087658592848
FPR(1.0) = 0.031625168768929485
FPR(2.0) = 0.6449551941586459
F1-Score(0.0) = 0.37107709398637495
F1-Score(1.0) = 0.08266995870759014
F1-Score(2.0) = 0.8189676817676388
Weighted precision: 0.6561208585718236
Weighted recall: 0.6959602962376064
Weighted F1 score: 0.6726804400193322
Weighted false positive rate: 0.49826153575111015
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.6977514074949597
Recall = 0.6977514074949597
F1 Score = 0.6977514074949597
Precision(0.0) = 0.27388629019168054                                            
Precision(1.0) = 0.15185504745470232
Precision(2.0) = 0.813411954147391
Recall(0.0) = 0.35740280746346254
Recall(1.0) = 0.05070730934339797
Recall(2.0) = 0.8334409601893331
FPR(0.0) = 0.14889676958642475
FPR(1.0) = 0.028270847952880002
FPR(2.0) = 0.6526511391703793
F1-Score(0.0) = 0.31012013166028973
F1-Score(1.0) = 0.07602755999049655
F1-Score(2.0) = 0.8233046608987815
Weighted precision: 0.680098934640914
Weighted recall: 0.6977514074949598
Weighted F1 score: 0.6857886690564517
Weighted false positive rate: 0.5275701642046438
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7502407047014238
Recall = 0.7502407047014238
F1 Score = 0.7502407047014238
Precision(0.0) = 0.3872559771879798                                             
Precision(1.0) = 0.19057537099713617
Precision(2.0) = 0.8238624935239082
Recall(0.0) = 0.3722196844583436
Recall(1.0) = 0.04454993609640314
Recall(2.0) = 0.8988960563942275
FPR(0.0) = 0.10048500908267936
FPR(1.0) = 0.017385323409514118
FPR(2.0) = 0.64375139229227
F1-Score(0.0) = 0.3795889846451544
F1-Score(1.0) = 0.07221783741120757
F1-Score(2.0) = 0.8597452573663873
Weighted precision: 0.7069367250170886
Weighted recall: 0.7502407047014238
Weighted F1 score: 0.7234929250778637
Weighted false positive rate: 0.5118624294858872
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.7393585219948646
Recall = 0.7393585219948646
F1 Score = 0.7393585219948646
Precision(0.0) = 0.339380708621901                                              
Precision(1.0) = 0.21537541130720908
Precision(2.0) = 0.82786180172205
Recall(0.0) = 0.34610266646194787
Recall(1.0) = 0.08495909376966645
Recall(2.0) = 0.8816913559932581
FPR(0.0) = 0.10518808558243602
FPR(1.0) = 0.02981370695501612
FPR(2.0) = 0.639111965520449
F1-Score(0.0) = 0.3427087292537691
F1-Score(1.0) = 0.12185146532028318
F1-Score(2.0) = 0.8539290998249139
Weighted precision: 0.708078974801972
Weighted recall: 0.7393585219948645
Weighted F1 score: 0.7205678496967879
Weighted false positive rate: 0.5134722800527657
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.749282610154372
Recall = 0.749282610154372
F1 Score = 0.749282610154372
Precision(0.0) = 0.3548667517861509                                             
Precision(1.0) = 0.2025189637898955
Precision(2.0) = 0.8367986790805102
Recall(0.0) = 0.3842058823529412
Recall(1.0) = 0.06610604998832048
Recall(2.0) = 0.8858667097765024
FPR(0.0) = 0.10826582295793462
FPR(1.0) = 0.024023040044148587
FPR(2.0) = 0.6172547604006858
F1-Score(0.0) = 0.3689539760771632
F1-Score(1.0) = 0.09967596506058042
F1-Score(2.0) = 0.8606338728082554
Weighted precision: 0.7185331922074465
Weighted recall: 0.749282610154372
Weighted F1 score: 0.7303573747593343
Weighted false positive rate: 0.49882623355714106
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.7313879774457647
Recall = 0.7313879774457647
F1 Score = 0.7313879774457647
Precision(0.0) = 0.35643726464006986                                            
Precision(1.0) = 0.1548327989005955
Precision(2.0) = 0.8417337478110959
Recall(0.0) = 0.4567771716323961
Recall(1.0) = 0.048921696338109714
Recall(2.0) = 0.8498204643258503
FPR(0.0) = 0.14763067292644758
FPR(1.0) = 0.021142739273927392
FPR(2.0) = 0.5497713019286085
F1-Score(0.0) = 0.4004169093528708
F1-Score(1.0) = 0.07435107787065552
F1-Score(2.0) = 0.8457577762168134
Weighted precision: 0.7176581871684279
Weighted recall: 0.7313879774457647
Weighted F1 score: 0.7215487928214213
Weighted false positive rate: 0.44993269157474813
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!



HEALTH 
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.7254314614767742
Recall = 0.7254314614767742
F1 Score = 0.7254314614767742
Precision(0.0) = 0.4715143505616686                                             
Precision(1.0) = 0.16955123296063715
Precision(2.0) = 0.7963703960427234
Recall(0.0) = 0.42293155579989006
Recall(1.0) = 0.046594831214748715
Recall(2.0) = 0.8824761656487412
FPR(0.0) = 0.11565593903778283
FPR(1.0) = 0.019859060009376466
FPR(2.0) = 0.5913732523241344
F1-Score(0.0) = 0.4459035397148123
F1-Score(1.0) = 0.07310067025456467
F1-Score(2.0) = 0.8372151566107293
Weighted precision: 0.6824780765224512
Weighted recall: 0.7254314614767742
Weighted F1 score: 0.6992981044878671
Weighted false positive rate: 0.4523197128480679
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7401137303322421
Recall = 0.7401137303322421
F1 Score = 0.7401137303322421
Precision(0.0) = 0.2611214135394745                                             
Precision(1.0) = 0.17040068935803532
Precision(2.0) = 0.8356977950844885
Recall(0.0) = 0.3114468909985586
Recall(1.0) = 0.05291323834370192
Recall(2.0) = 0.8736730510990176
FPR(0.0) = 0.11333810622670817
FPR(1.0) = 0.023829118427810332
FPR(2.0) = 0.6930392380517851
F1-Score(0.0) = 0.284072491527921
F1-Score(1.0) = 0.08075136542289826
F1-Score(2.0) = 0.8542635953553701
Weighted recall: 0.7401137303322421
Weighted F1 score: 0.7237970679640032
Weighted false positive rate: 0.5703201930385458
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7706817793745969
Recall = 0.7706817793745969
F1 Score = 0.7706817793745969
Precision(0.0) = 0.21201163612762652                                            
Precision(1.0) = 0.1319718309859155
Precision(2.0) = 0.8648585541677355
Recall(0.0) = 0.2872464041203442
Recall(1.0) = 0.03720394671537194
Recall(2.0) = 0.8846001184037028
FPR(0.0) = 0.10541951509193778
FPR(1.0) = 0.01872512381125999
FPR(2.0) = 0.7205821752663188
F1-Score(0.0) = 0.24396033794101368
F1-Score(1.0) = 0.058044633039599815
F1-Score(2.0) = 0.8746179505855043
Weighted precision: 0.7540926685913808
Weighted recall: 0.7706817793745968
Weighted F1 score: 0.7598975756911567
Weighted false positive rate: 0.6154085935441137
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.7617855851397902
Recall = 0.7617855851397902
F1 Score = 0.7617855851397902
Precision(0.0) = 0.4605596223575289                                             
Precision(1.0) = 0.24852489969317915
Precision(2.0) = 0.8239285572803776
Recall(0.0) = 0.3895946063254145
Recall(1.0) = 0.06578782956391353
Recall(2.0) = 0.9121717719147656
FPR(0.0) = 0.08979973008831921
FPR(1.0) = 0.016398339565114387
FPR(2.0) = 0.615287254029467
F1-Score(0.0) = 0.42211527910585805
F1-Score(1.0) = 0.10403596304895518
F1-Score(2.0) = 0.8658075335704177
Weighted precision: 0.7203582531231186
Weighted recall: 0.7617855851397903
Weighted F1 score: 0.7348363462580866
Weighted false positive rate: 0.4832709088226909
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Game
s
Summary Statistics                                                              
Precision = 0.7002575022283847
Recall = 0.7002575022283847
F1 Score = 0.7002575022283847
Precision(0.0) = 0.3843691210931054                                             
Precision(1.0) = 0.17237533853751794
Precision(2.0) = 0.7890128814493352
Recall(0.0) = 0.377039627039627
Recall(1.0) = 0.062471131639722864
Recall(2.0) = 0.8577408677679762
FPR(0.0) = 0.12364607776849752
FPR(1.0) = 0.031594759952805515
FPR(2.0) = 0.6353509790906073
F1-Score(0.0) = 0.38066909637668134
F1-Score(1.0) = 0.09170657286943255
F1-Score(2.0) = 0.8219426783587124
Weighted precision: 0.6614788575196978
Weighted recall: 0.7002575022283847
Weighted F1 score: 0.6773576654982627
Weighted false positive rate: 0.49084931904029505
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7208989140127139
Recall = 0.7208989140127139
F1 Score = 0.7208989140127139
Precision(0.0) = 0.3064010203026438                                             
Precision(1.0) = 0.16265124745690115
Precision(2.0) = 0.8137823117160123
Recall(0.0) = 0.34232568886834963
Recall(1.0) = 0.04376386527989858
Recall(2.0) = 0.866831206153326
FPR(0.0) = 0.12177291487636316
FPR(1.0) = 0.022490135400968628
FPR(2.0) = 0.6771427252371829
F1-Score(0.0) = 0.32336865081169575
F1-Score(1.0) = 0.06897021431165999
F1-Score(2.0) = 0.83946950956975
Weighted precision: 0.6857808350129895
Weighted recall: 0.7208989140127139
Weighted F1 score: 0.6994497773481304
Weighted false positive rate: 0.5423046895272285
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7646317730205879
Recall = 0.7646317730205879
F1 Score = 0.7646317730205879
Precision(0.0) = 0.4346620589889898                                             
Precision(1.0) = 0.2203881329466875
Precision(2.0) = 0.8288394186544177
Recall(0.0) = 0.38009065673424924
Recall(1.0) = 0.0601302416164567
Recall(2.0) = 0.9143911684511539
FPR(0.0) = 0.08434601711020917
FPR(1.0) = 0.01954381000844382
FPR(2.0) = 0.6325239474270439
F1-Score(0.0) = 0.4055487862030181
F1-Score(1.0) = 0.09448216505689969
F1-Score(2.0) = 0.8695160010244704
Weighted precision: 0.7201875874847867
Weighted recall: 0.7646317730205879
Weighted F1 score: 0.7366745387414279
Weighted false positive rate: 0.5010455475662848
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.7520104505413615
Recall = 0.7520104505413615
F1 Score = 0.7520104505413615
Precision(0.0) = 0.3665906636265451                                             
Precision(1.0) = 0.27577937649880097
Precision(2.0) = 0.8406139763057744
Recall(0.0) = 0.3908593070269717
Recall(1.0) = 0.11308212712397735
Recall(2.0) = 0.8870146446026657
FPR(0.0) = 0.10544379407475478
FPR(1.0) = 0.028605094358923843
FPR(2.0) = 0.5863074013208893
F1-Score(0.0) = 0.3783362025191039
F1-Score(1.0) = 0.16039499009735278
F1-Score(2.0) = 0.8631911956272423
Weighted precision: 0.7269704286567265
Weighted recall: 0.7520104505413615
Weighted F1 score: 0.7359632703221006
Weighted false positive rate: 0.4723667402959295
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.7537823318821073
Recall = 0.7537823318821073
F1 Score = 0.7537823318821073
Precision(0.0) = 0.37104132057062994                                            
Precision(1.0) = 0.23615274338589862
Precision(2.0) = 0.8427652067599505
Recall(0.0) = 0.4138529411764706
Recall(1.0) = 0.0846531184302733
Recall(2.0) = 0.8845279472982258
FPR(0.0) = 0.10873995322522556
FPR(1.0) = 0.02526903045562722
FPR(2.0) = 0.5895857774569082
F1-Score(0.0) = 0.39127956286584265
F1-Score(1.0) = 0.12463030469770962
F1-Score(2.0) = 0.8631417042768371
Weighted precision: 0.7282072179423176
Weighted recall: 0.7537823318821073
Weighted F1 score: 0.7374212581098302
Weighted false positive rate: 0.4773770930198683
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.730602189587249
Recall = 0.730602189587249
F1 Score = 0.730602189587249
Precision(0.0) = 0.35972229418164864                                            
Precision(1.0) = 0.19546436285097193
Precision(2.0) = 0.8505146059311455
Recall(0.0) = 0.48559239054413206
Recall(1.0) = 0.07859313938341293
Recall(2.0) = 0.8403503001397912
FPR(0.0) = 0.154716744913928
FPR(1.0) = 0.025611936193619362
FPR(2.0) = 0.5081812609044184
F1-Score(0.0) = 0.41328610970564605
F1-Score(1.0) = 0.11210901207804273
F1-Score(2.0) = 0.8454019026609679
Weighted precision: 0.7279413566682438
Weighted recall: 0.730602189587249
Weighted F1 score: 0.7259970606286167
Weighted false positive rate: 0.41911213159921473
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!

Clothing 
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.6991141646056701
Recall = 0.6991141646056701
F1 Score = 0.6991141646056701
Precision(0.0) = 0.4296473255861036                                             
Precision(1.0) = 0.13857677902621723
Precision(2.0) = 0.7734415010722236
Recall(0.0) = 0.273441794942276
Recall(1.0) = 0.08565535819513427
Recall(2.0) = 0.8823039252197229
FPR(0.0) = 0.08856371607970692
FPR(1.0) = 0.0463329231129864
FPR(2.0) = 0.6773357245687236
F1-Score(0.0) = 0.3341924443721228
F1-Score(1.0) = 0.10587102983638115
F1-Score(2.0) = 0.8242939542368182
Weighted precision: 0.6551907734908168
Weighted recall: 0.6991141646056702
Weighted F1 score: 0.6706588937408656
Weighted false positive rate: 0.5113465283670872
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7459899862934559
Recall = 0.7459899862934559
F1 Score = 0.7459899862934559
Precision(0.0) = 0.23640986184056467                                            
Precision(1.0) = 0.1343661081251976
Precision(2.0) = 0.8199542133682797
Recall(0.0) = 0.17563000149112779
Recall(1.0) = 0.056859990634825074
Recall(2.0) = 0.8999010530779561
FPR(0.0) = 0.07295495368801898
FPR(1.0) = 0.03388425149589441
FPR(2.0) = 0.7972653131059656
F1-Score(0.0) = 0.2015371233833825
F1-Score(1.0) = 0.0799059929494712
F1-Score(2.0) = 0.8580694834984695
Weighted precision: 0.6954105201135705
Weighted recall: 0.7459899862934561
Weighted F1 score: 0.7173704465056829
Weighted false positive rate: 0.650094504583335
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.7749548072268924
Recall = 0.7749548072268924
F1 Score = 0.7749548072268924
Precision(0.0) = 0.19228657471340865                                            
Precision(1.0) = 0.1228655796636282
Precision(2.0) = 0.8553460628542088
Recall(0.0) = 0.18147415363356573
Recall(1.0) = 0.05699708165412638
Recall(2.0) = 0.8993450795188505
FPR(0.0) = 0.07527130136274764
FPR(1.0) = 0.03113663294139094
FPR(2.0) = 0.7928806277673053
F1-Score(0.0) = 0.18672396939904837
F1-Score(1.0) = 0.07787029753993871
F1-Score(2.0) = 0.8767939318066108
Weighted precision: 0.7436912596328547
Weighted recall: 0.7749548072268925
Weighted F1 score: 0.7579888021021387
Weighted false positive rate: 0.6742433692983362
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.7147479207506233
Recall = 0.7147479207506233
F1 Score = 0.7147479207506233
Precision(0.0) = 0.3896454151560704                                             
Precision(1.0) = 0.1397863470557582
Precision(2.0) = 0.8087072159440657
Recall(0.0) = 0.2550131658902167
Recall(1.0) = 0.13407472197925777
Recall(2.0) = 0.872524388028094
FPR(0.0) = 0.0786103534476377
FPR(1.0) = 0.06801396742993109
FPR(2.0) = 0.6514585187382577
F1-Score(0.0) = 0.30827080819210523
F1-Score(1.0) = 0.1368709739141527
F1-Score(2.0) = 0.8394045972231011
Weighted precision: 0.6888572635200578
Weighted recall: 0.7147479207506233
Weighted F1 score: 0.6985665893542831
Weighted false positive rate: 0.5128307603664497
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6973798598043424
Recall = 0.6973798598043424
F1 Score = 0.6973798598043424
Precision(0.0) = 0.3675277144221079                                             
Precision(1.0) = 0.1489460273337966
Precision(2.0) = 0.7683895267050869
Recall(0.0) = 0.22432659932659932
Recall(1.0) = 0.07424942263279445
Recall(2.0) = 0.8876200032949423
FPR(0.0) = 0.07904121756883957
FPR(1.0) = 0.04468879617578728
FPR(2.0) = 0.741121805509459
F1-Score(0.0) = 0.2786031643915482
F1-Score(1.0) = 0.09909840487015487
F1-Score(2.0) = 0.8237125473858309
Weighted precision: 0.6412308488419844
Weighted recall: 0.6973798598043424
Weighted F1 score: 0.6620162483184572
Weighted false positive rate: 0.5622316790584282
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7265001294398523
Recall = 0.7265001294398523
F1 Score = 0.7265001294398523
Precision(0.0) = 0.2967798085291558                                             
Precision(1.0) = 0.14899771290192385
Precision(2.0) = 0.7984767964522854
Recall(0.0) = 0.20355072882367667
Recall(1.0) = 0.06381630124751506
Recall(2.0) = 0.896086552277914
FPR(0.0) = 0.07579186889531717
FPR(1.0) = 0.036383977360313825
FPR(2.0) = 0.7720505066826712
F1-Score(0.0) = 0.24147934941520469
F1-Score(1.0) = 0.08935955622793747
F1-Score(2.0) = 0.8444704296749916
Weighted precision: 0.6713971969973411
Weighted recall: 0.7265001294398523
Weighted F1 score: 0.6940475167877368
Weighted false positive rate: 0.6107264823781545
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.7565963330943357
Recall = 0.7565963330943357
F1 Score = 0.7565963330943357
Precision(0.0) = 0.42309876932786367                                            
Precision(1.0) = 0.19236270022883295
Precision(2.0) = 0.8101239393816371
Recall(0.0) = 0.23556695597174884
Recall(1.0) = 0.08185746454871888
Recall(2.0) = 0.9289352929440713
FPR(0.0) = 0.054801829725241454
FPR(1.0) = 0.031577652394186626
FPR(2.0) = 0.7293161060369793
F1-Score(0.0) = 0.3026363308053449
F1-Score(1.0) = 0.11484438372539811
F1-Score(2.0) = 0.865471060400938
Weighted precision: 0.70173110810498
Weighted recall: 0.7565963330943357
Weighted F1 score: 0.720273577588192
Weighted false positive rate: 0.5722919212507431
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.7899351333791812
Recall = 0.7899351333791812
F1 Score = 0.7899351333791812
Precision(0.0) = 0.527120315581854                                              
Precision(1.0) = 0.31091058244462677
Precision(2.0) = 0.8460448280998989
Recall(0.0) = 0.3556220891550233
Recall(1.0) = 0.17888609188168658
Recall(2.0) = 0.9345017588643652
FPR(0.0) = 0.04981121521465529
FPR(1.0) = 0.03819064253482812
FPR(2.0) = 0.5928188273231838
F1-Score(0.0) = 0.42471195868096945
F1-Score(1.0) = 0.22710476380705083
F1-Score(2.0) = 0.8880760388139433
Weighted precision: 0.7559566510982788
Weighted recall: 0.7899351333791811
Weighted F1 score: 0.7674252464900747
Weighted false positive rate: 0.4707558184518484
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.7524837279799802
Recall = 0.7524837279799802
F1 Score = 0.7524837279799802
Precision(0.0) = 0.38054486927848                                               
Precision(1.0) = 0.20497549943460233
Precision(2.0) = 0.830473882857276
Recall(0.0) = 0.28511764705882353
Recall(1.0) = 0.1270263957019388
Recall(2.0) = 0.9003960716162147
FPR(0.0) = 0.07194015017164428
FPR(1.0) = 0.04546787155520298
FPR(2.0) = 0.6566555365039256
F1-Score(0.0) = 0.3259911894273128
F1-Score(1.0) = 0.15685030285549467
F1-Score(2.0) = 0.8640226491562317
Weighted precision: 0.7172451771633858
Weighted recall: 0.7524837279799802
Weighted F1 score: 0.7320699131937827
Weighted false positive rate: 0.526547286210753
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.716744714514776
Recall = 0.716744714514776
F1 Score = 0.716744714514776
Precision(0.0) = 0.3437523480351642                                             
Precision(1.0) = 0.14205483977535513
Precision(2.0) = 0.8296083411308649
Recall(0.0) = 0.3199748216533781
Recall(1.0) = 0.1244753220437111
Recall(2.0) = 0.8505742400570129
FPR(0.0) = 0.10934585289514867
FPR(1.0) = 0.05952053538687202
FPR(2.0) = 0.6010751167067477
F1-Score(0.0) = 0.33143767884956715
F1-Score(1.0) = 0.1326853351847566
F1-Score(2.0) = 0.8399604807275878
Weighted precision: 0.7053999573037856
Weighted recall: 0.7167447145147761
Weighted F1 score: 0.710863786326779
Weighted false positive rate: 0.4866862195035444
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!


Music 
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Electronics
Summary Statistics                                                              
Precision = 0.647827361497665
Recall = 0.647827361497665
F1 Score = 0.647827361497665
Precision(0.0) = 0.3619918867455915                                             
Precision(1.0) = 0.11977181921060533
Precision(2.0) = 0.7568433000281686
Recall(0.0) = 0.07511854040681694
Recall(1.0) = 0.21828436737099083
Recall(2.0) = 0.850518583345747
FPR(0.0) = 0.032302346441774876
FPR(1.0) = 0.13959578645100798
FPR(2.0) = 0.716138398848303
F1-Score(0.0) = 0.12441845575995562
F1-Score(1.0) = 0.15467438149633894
F1-Score(2.0) = 0.8009512954276445
Weighted precision: 0.6284020357142415
Weighted recall: 0.6478273614976648
Weighted F1 score: 0.6165268005035697
Weighted false positive rate: 0.5358638932387508
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Books
Summary Statistics                                                              
Precision = 0.7539363835113674
Recall = 0.7539363835113674
F1 Score = 0.7539363835113674
Precision(0.0) = 0.286765382139244                                              
Precision(1.0) = 0.1673854534842245
Precision(2.0) = 0.8283355384002774
Recall(0.0) = 0.07748894080222675
Recall(1.0) = 0.1726536892099806
Recall(2.0) = 0.9115379178740547
FPR(0.0) = 0.024786018831621272
FPR(1.0) = 0.07944173901205998
FPR(2.0) = 0.7621906011178282
F1-Score(0.0) = 0.1220089608890454
F1-Score(1.0) = 0.1699787608871034
F1-Score(2.0) = 0.8679473202508816
Weighted precision: 0.7106609340593482
Weighted recall: 0.7539363835113674
Weighted F1 score: 0.7238503898034939
Weighted false positive rate: 0.6203547424728769
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/2_Music
Summary Statistics                                                              
Precision = 0.8147893614589258
Recall = 0.8147893614589258
F1 Score = 0.8147893614589258
Precision(0.0) = 0.3348719570028454                                             
Precision(1.0) = 0.18686450697564436
Precision(2.0) = 0.8585443652653175
Recall(0.0) = 0.08316060548960492
Recall(1.0) = 0.12550872525858134
Recall(2.0) = 0.9515469847420683
FPR(0.0) = 0.016309867322431146
FPR(1.0) = 0.041791997083219394
FPR(2.0) = 0.8172986716934812
F1-Score(0.0) = 0.13323438030667054
F1-Score(1.0) = 0.1501609206322815
F1-Score(2.0) = 0.9026564344746163
Weighted precision: 0.7637379853726846
Weighted recall: 0.8147893614589258
Weighted F1 score: 0.7800202167175838
Weighted false positive rate: 0.6901898975580576
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Health
Summary Statistics                                                              
Precision = 0.681037436004796
Recall = 0.681037436004796
F1 Score = 0.681037436004796
Precision(0.0) = 0.30284770142871026                                            
Precision(1.0) = 0.13908311345646437
Precision(2.0) = 0.800894062973644
Recall(0.0) = 0.09016464596776527
Recall(1.0) = 0.26346370111208295
Recall(2.0) = 0.8508524062227847
FPR(0.0) = 0.04084549549293048
FPR(1.0) = 0.1344365130867402
FPR(2.0) = 0.6676752694551568
F1-Score(0.0) = 0.1389582590082055
F1-Score(1.0) = 0.1820575918490696
F1-Score(2.0) = 0.8251177203268828
Weighted precision: 0.6685979899163226
Weighted recall: 0.681037436004796
Weighted F1 score: 0.6633178362313418
Weighted false positive rate: 0.5239947140396235
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Video_Games
Summary Statistics                                                              
Precision = 0.6884443123920196
Recall = 0.6884443123920196
F1 Score = 0.6884443123920196
Precision(0.0) = 0.34838005096468877                                            
Precision(1.0) = 0.1580020387359837
Precision(2.0) = 0.766527427541114
Recall(0.0) = 0.09294871794871795
Recall(1.0) = 0.16108545034642033
Recall(2.0) = 0.8945843130794231
FPR(0.0) = 0.03559638865688263
FPR(1.0) = 0.09042365562623916
FPR(2.0) = 0.7547709923664122
F1-Score(0.0) = 0.14674538066395768
F1-Score(1.0) = 0.15952884670364229
F1-Score(2.0) = 0.8256198489900997
Weighted precision: 0.6374715148839031
Weighted recall: 0.6884443123920196
Weighted F1 score: 0.6467671053959666
Weighted false positive rate: 0.5692353490415537
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Movies
Summary Statistics                                                              
Precision = 0.7470065399812247
Recall = 0.7470065399812247
F1 Score = 0.7470065399812247
Precision(0.0) = 0.3898394314293235                                             
Precision(1.0) = 0.17789119880492968
Precision(2.0) = 0.8027960900204592
Recall(0.0) = 0.11407005179750833
Recall(1.0) = 0.12351263361087902
Recall(2.0) = 0.9313058913025104
FPR(0.0) = 0.028055821159269436
FPR(1.0) = 0.05697884431764584
FPR(2.0) = 0.780972276724914
F1-Score(0.0) = 0.17649600023834705
F1-Score(1.0) = 0.1457964902734322
F1-Score(2.0) = 0.8622892265889495
Weighted precision: 0.6899980135233023
Weighted recall: 0.7470065399812247
Weighted F1 score: 0.7041266814906899
Weighted false positive rate: 0.613013482183054
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Toys
Summary Statistics                                                              
Precision = 0.730246850353375
Recall = 0.730246850353375
F1 Score = 0.730246850353375
Precision(0.0) = 0.33189655172413796                                            
Precision(1.0) = 0.16832080775629626
Precision(2.0) = 0.8025190710487764
Recall(0.0) = 0.07575810815559225
Recall(1.0) = 0.17856490779623882
Recall(2.0) = 0.9143978187138392
FPR(0.0) = 0.026019028662897705
FPR(1.0) = 0.0810662700121345
FPR(2.0) = 0.753731343283582
F1-Score(0.0) = 0.12335860391932485
F1-Score(1.0) = 0.17329159529856475
F1-Score(2.0) = 0.8548132905195165
Weighted precision: 0.6805588234731406
Weighted recall: 0.7302468503533749
Weighted F1 score: 0.6908547127251382
Weighted false positive rate: 0.5910634923119893
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Clothing
Summary Statistics                                                              
Precision = 0.688581470333111
Recall = 0.688581470333111
F1 Score = 0.688581470333111
Precision(0.0) = 0.24206590731240762                                            
Precision(1.0) = 0.16231640417625198
Precision(2.0) = 0.8129153163066184
Recall(0.0) = 0.07124213112237064
Recall(1.0) = 0.28862492133417245
Recall(2.0) = 0.8410884946700407
FPR(0.0) = 0.03482829574285315
FPR(1.0) = 0.14348012230098622
FPR(2.0) = 0.6748007813711203
F1-Score(0.0) = 0.11008521323078747
F1-Score(1.0) = 0.20778117567108392
F1-Score(2.0) = 0.8267619640886091
Weighted precision: 0.6786601421942466
Weighted recall: 0.688581470333111
Weighted F1 score: 0.6755910761908852
Weighted false positive rate: 0.5416906697480707
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Sports
Summary Statistics                                                              
Precision = 0.6913743492178773
Recall = 0.6913743492178773
F1 Score = 0.6913743492178773
Precision(0.0) = 0.24241102581995813                                            
Precision(1.0) = 0.1508096350600177
Precision(2.0) = 0.8148901029094143
Recall(0.0) = 0.08173529411764706
Recall(1.0) = 0.2623686054660126
Recall(2.0) = 0.8424807016125773
FPR(0.0) = 0.03959443626367114
FPR(1.0) = 0.13633894388300624
FPR(2.0) = 0.6837289053334537
F1-Score(0.0) = 0.12225057188104874
F1-Score(1.0) = 0.19152854511970532
F1-Score(2.0) = 0.8284557490250627
Weighted precision: 0.6819551750614344
Weighted recall: 0.6913743492178773
Weighted F1 score: 0.6798686110356069
Weighted false positive rate: 0.5510366346980083
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!! /lustre/scratch/riomus/Neurocomputing_2016/Automotive
Summary Statistics                                                              
Precision = 0.669342592887558
Recall = 0.669342592887558
F1 Score = 0.669342592887558
Precision(0.0) = 0.2524936436534324                                             
Precision(1.0) = 0.12943632567849686
Precision(2.0) = 0.8104893397710627
Recall(0.0) = 0.090292348580221
Recall(1.0) = 0.28716167317991026
Recall(2.0) = 0.8189978894279527
FPR(0.0) = 0.047849765258215965
FPR(1.0) = 0.15291529152915292
FPR(2.0) = 0.6588862168152025
F1-Score(0.0) = 0.1330173612899902
F1-Score(1.0) = 0.17844133651122004
F1-Score(2.0) = 0.8147214004280904
Weighted precision: 0.6758051124717793
Weighted recall: 0.669342592887558
Weighted F1 score: 0.6645396783506562
Weighted false positive rate: 0.5289938664901295
!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
